A quantum fluctuation description of charge qubits

We consider a specific instance of a superconducting circuit, the so-called charge-qubit, consisting of a capacitor and a Josephson junction. Starting from the microscopic description of the latter in terms of two tunneling BCS models in the strong-coupling quasi-spin formulation, we derive the Hamiltonian governing the quantum behavior of the circuit in the limit of a large number $N$ of quasi-spins. Our approach relies on the identification of suitable quantum fluctuations, i.e. of collective quasi-spin operators, which account for the presence of fluctuation operators in the superconducting phase that retain a quantum character in spite of the large-$N$ limit. We show indeed that these collective quantum fluctuations generate the Heisenberg algebra on the circle and that their dynamics reproduces the one of the quantized charge-qubit, without the need of a phenomenological ``third quantization'' of a semiclassically inspired model. As a byproduct of our derivation, we explicitly obtain the temperature dependence of the junction critical Josephson current in the strong coupling regime, a result which is not directly accessible using standard approximation techniques.

==> packages.tex <==
\usepackage{comment}
\usepackage{appendix}


%MATEMATICA I pacchetti amsmath e amssymb sono i due fondamentali per scrivere matematica. Il pacchetto amsthm serve per l'utilizzo di enunciati (definizioni, teoremi, dimostrazioni...), mentre mathtools serve per definire dei nuovi tipi di parentesi come il valore assoluto e la norma.
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{thmtools,thm-restate}
\usepackage{amsfonts}
\usepackage{mathtools}

%\usepackage[output-decimal-marker={.}, separate-uncertainty]{siunitx}
\usepackage{braket}

\usepackage{chemformula}

\usepackage{circuitikz}
\usepackage{pgfplots}
\pgfplotsset{/pgf/number format/use comma,compat=newest}

\usepackage{subfig}





